SapientML: Synthesizing Machine Learning Pipelines by Learning from Human-Written Solutions

Automatic machine learning, or AutoML, holds the promise of truly democratizing the use of machine learning (ML), by substantially automating the work of data scientists. However, the huge combinatorial search space of candidate pipelines means that current AutoML techniques, generate sub-optimal pipelines, or none at all, especially on large, complex datasets. In this work we propose an AutoML technique SapientML, that can learn from a corpus of existing datasets and their human-written pipelines, and efficiently generate a high-quality pipeline for a predictive task on a new dataset. To combat the search space explosion of AutoML, SapientML employs a novel divide-and-conquer strategy realized as a three-stage program synthesis approach, that reasons on successively smaller search spaces. The first stage uses a machine-learned model to predict a set of plausible ML components to constitute a pipeline. In the second stage, this is then refined into a small pool of viable concrete pipelines using syntactic constraints derived from the corpus and the machine-learned model. Dynamically evaluating these few pipelines, in the third stage, provides the best solution. We instantiate SapientML as part of a fully automated tool-chain that creates a cleaned, labeled learning corpus by mining Kaggle, learns from it, and uses the learned models to then synthesize pipelines for new predictive tasks. We have created a training corpus of 1094 pipelines spanning 170 datasets, and evaluated SapientML on a set of 41 benchmark datasets, including 10 new, large, real-world datasets from Kaggle, and against 3 state-of-the-art AutoML tools and 2 baselines. Our evaluation shows that SapientML produces the best or comparable accuracy on 27 of the benchmarks while the second best tool fails to even produce a pipeline on 9 of the instances.

==> algorithm-pipeline-instantiation.tex <==
\begin{algorithm}[t]\scriptsize
\caption{Algorithm for Pipeline Instantiation}
\label{alg:pipeline-instantiation}
\begin{flushleft}
\textbf{Input:} \hspace*{0.5em} $\mathcal{D}$: User dataset \\
\hspace*{3.5em} $\mathcal{C}_{p}$: Set of pre-processing components from pipeline skeleton \\
\hspace*{3.5em} $\mathcal{C}_{m}$: Set of model components from pipeline skeleton \\
\hspace*{3.5em} $\mathcal{G}$: DAG of relative component ordering mined from our data corpus \\
\hspace*{3.5em} $\mathcal{M}$: Dictionary of top-K hyperparameters mined from our data corpus for $m \in \mathcal{C}_{m}$\\
\textbf{Output:} $\mathcal{P}_{\mathit{best}}$: Best pipeline synthesized for $\mathcal{D}$ \\
$\textbf{begin}$
\end{flushleft}
\begin{algorithmic}[1]

\State \highlightgray{/* Step 1. Infer target columns */}
\For {\textbf{each} $c_{p}$ $\in$ $\mathcal{C}_{p}$}
    \State \textit{relevantColumns} $\gets$ \{\}
    \For {\textbf{each} $col$ $\in$ $\mathcal{D}$.\textit{columns}}
        \For {\textbf{each} \textit{pred} $\in$ $c_{p}$.\textit{target\_predicates}}
            \If {\textit{pred}($col$) = \textit{TRUE}}
                \State \textit{relevantColumns} $\gets$ \textit{relevantColumns} $\cup$ $col$
                \State \textbf{break}
            \EndIf
        \EndFor
    \EndFor
    \State $c$.\textit{target\_columns} $\gets$ \textit{relevantColumns}
\EndFor

\State \highlightgray{/* Step 2. Partial ordering of pre-processing components */}
\State $\mathcal{G}_{p}$ $\gets$
\textsc{ConstructDAG}($\mathcal{C}_{p}$, $\mathcal{G}$)

\State \highlightgray{/* Step 3. Discard redundant components */}
\State \textit{level\_nodes} $\gets$ \textsc{GetNodesAtEachLevel}($\mathcal{G}_{p}$)
\For {\textbf{each} $N$ $\in$ \textit{level\_nodes}}
    \State \textit{groups} $\gets$ \textsc{GroupByTargetColumns}($N$)
    \For {\textbf{each} $g$ $\in$ \textit{groups}}
        \State $g$ $\gets$ \textsc{SortByProbability}($g$)
        \For {$i$ $\gets$ 2 to $g$.size()}
            \State \textsc{RemoveNode}($g$[$i$], $\mathcal{G}_{p}$)
        \EndFor
    \EndFor
\EndFor

\State \highlightgray{/* Step 4. Total ordering of pre-processing components */}
\State $\mathcal{L}_{p}$ $\gets$ \textsc{TopologicalSort}($\mathcal{G}_{p}$)

\State \highlightgray{/* Step 5. Build candidates and select best pipeline */}
\For {\textbf{each} $c$ $\in$ $\mathcal{L}_{p}$}
    \State $\mathcal{P}_\textit{preprocess}$ $\gets$ $\mathcal{P}_\textit{preprocess}$ $\biguplus$ \textsc{InstantiateTemplate}($c$)
\EndFor

\State \textit{max\_score} $\gets$ 0
\For {\textbf{each} $m$ $\in$ $\mathcal{C}_{m}$}
    \For {\textbf{each} $hp$ $\in$ $\mathcal{M}$[$m$]}
        \State $\mathcal{P}$ $\gets$ $\mathcal{P}_\textit{preprocess}$ $\biguplus$ \textsc{InstantiateTemplate}($m$, $hp$)
        \State \textit{score} $\gets$ \textsc{RunPipeline}($\mathcal{P}$)
         \If {\textit{score} $>$ \textit{max\_score}}
            \State \textit{max\_score} $\gets$ \textit{score}
            \State $\mathcal{P}_{\mathit{best}}$ $\gets$ $\mathcal{P}$
         \EndIf
     \EndFor
\EndFor

\State \Return $\mathcal{P}_{\mathit{best}}$

\end{algorithmic}
\begin{flushleft}
\textbf{end}
\end{flushleft}
\end{algorithm}


==> experimental-setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

\subsection{Implementation}
\label{sec:implementation}

\tool{} is implemented in Python programming language.   It includes a crawler to download ML projects, a set of tools for required static and dynamic analysis such as mining order of ML components from corpus, denoising pipelines and datasets, a meta-feature extractor, and machine learning models for skeleton predictor. \tool uses Kaggle Public APIs~\cite{kaggleapi} for automatically downloading data, Python-PL libraries~\cite{pythonpl} to instrument source code for dynamic program slicing, the scikit-learn~\cite{} library to implement meta-models for the skeleton predictor, and LibCST~\cite{libCST} for static analysis. \tool uses Pandas and Numpy for computing meta-features and its own data analysis. The total size of the \tool{} code-base is approximately \ripon{X} lines of code.

\subsection{Benchmarks}
\label{sec:benchmarks}

We use a set of \numBM{} benchmark datasets to evaluate \tool. This includes the set of 31 benchmarks used in \cite{AL:OOPSLA2019}, which contains 12 datasets from the OpenML suite, 9 from PMLB, 4 from Mulan, and 6 from Kaggle. They were collectively used to benchmark AL~\cite{AL:OOPSLA2019} against TPOT~\cite{TPOT:GECCO2016}
and \autosk~\cite{Auto-sklearn-NIPS2015}. However, one of the limitations of the these benchmark datasets is that most of them are small and simple in nature. To overcome this limitation, we have added \numNewBM{} new datasets from Kaggle as representatives of large, real-world datasets which modern AutoML tools should handle.

In order to scientifically select these \numNewBM{} new benchmark datasets first we list all the {\it Featured} and {\it Playground} competitions on Kaggle that completed since the year of 2015. Second, we examine each dataset and exclude the ones that contain non-tabular data. Third, we check the dataset licenses and keep only those dataset that allows academic research and using dataset outside of the competition. Finally, we selected \numNewBM{} datasets based on size either in terms of large number of rows or columns, or have various types of columns.

\subsection{Research Questions}
\label{sec:rqs}

Our evaluation addresses the following research questions:
\begin{itemize}
    \item[\textbf{RQ1:}] How does \tool perform compared to the existing state-of-the-art techniques? 
    \item[\textbf{RQ2:}] How robust \tool{} is in producing good quality pipelines across trials?
    \item[\textbf{RQ3:}] Does \tool{} predict a diverse set of pre-processing and model components?
    % \item[\textbf{RQ2:}] How efficient is \tool in its pipeline generation? 
    \item[\textbf{RQ4:}] Does each of the novel technology components of \tool contribute to its effectiveness?
\end{itemize}

\subsection{Methodology}

\tool{} is trained on the meta-training data extracted from our ML project corpus. Therefore, the 41 benchmark datasets are completely unseen to \tool{}. We performed 10 trials of each experiment for each benchmark with one hour time out \ripon{discuss}. \ura{FYI: I set time limit to 3600 seconds for autosklearn and tpot, but execution time of some experiments was over 3600 seconds. I regarded them as succeeded.} For each trial, we randomly split the data into training and testing data in a 75:25 split.\ura{I think the current description is sufficient, but I can add "For each trial, we generated a pipeline using only the training data and then evaluated it using the test data." to avoid misunderstanding in the FSE review.} All the baselines and existing tools were run using the same train-test split of data in each trial to ensure a fare comparison. We use standard {\it macro} F1 scores and $R^2$ scores for classification and regression tasks respectively, and used the mean score of 10 runs to compare the results, following existing literature~\cite{}.

\subsection{Experimental Configurations}
We ran all tools on 4 vCPUs of Xeon E5-2697A v4 (2.60GHz) with 16GB memory for \openml, PMLB, and \mulan datasets and on 8 vCPUs with 32GB memory for Kaggle datasets.

==> formulation.tex <==
\subsection{Approach Formulation}
\label{appsec:formulation}

\begin{definition}[Dataset]
\label{def:dataset}
A dataset, $d \in D$ is comprised of a number of $n$ rows and $\{m \cup t\}$ columns where each row represents an observation consisting of $m$ values from an input domain $x \in X$ and $t$ values from an output domain $y \in Y$. 
\end{definition}

\begin{definition}[Predictive Task]
\label{def:task}
A supervised predictive task is to learn a prediction function $f : X \xrightarrow{} Y$ such that $\hat y \approx f(x)$. A predictive task is called a {\it classification} task when the $y$ is discrete and called a {\it regression} task when $y$ is continuous. For multi-label classification and multivariate regression, $|t|>1$.
\end{definition}

\begin{definition}[Component]
\label{def:component}
A component $c \in C$ is one API or a set of APIs, and associated glue code required to instantiate them, that performs a specific atomic task, \eg filling missing values or transforming a categoric column to a set of numeric columns. There are mainly two kinds of components: i) the pre-processing component that transforms data from one property to another property, and ii) the model component that performs the actual learning and prediction. 
\end{definition}

\begin{definition}[Pipeline]
\label{def:pipeline}
Given a dataset $d$, a pipeline ($\rho \in \mathbb{P}$) is a sequence of pre-processing components followed by a model component that realizes a given predictive task.
\end{definition}

\begin{definition}[Entity]
\label{def:entity}
An entity $e$ refers to a component of a dataset $d$, specifically a row, a column, a cell in a row of $d$ or the entire dataset $d$. Each entity $e$ is associated with a set of properties $\mathcal{P}(e) = \{ p_1, p_2, \ldots, p_k \}$ describing the shape, type, distribution of values, \etc of $e$.
\end{definition}

\mukul{@Ripon please add a table showing the list of properties associated with different entities.}


\begin{table}[t]
 \centering
 \footnotesize
 \caption{List of Components}
 \label{tbl:components}
 \begin{tabular}{l|ll}
 \hline
 Preprocessing & \multicolumn{2}{c}{Models (Classifiers and Regressors)}\\
 \hline \hline
SimpleImputer & RandomForest & SVM\\
LabelEncoder & ExtraTrees & LinearSVM\\
OneHotEncoder& LightGBM & LogisticRegression\\
StringVectorizer & XGBosst & Lasso\\
TextPreprocessing & CatBoost & SGD\\
DateProcessing & GradientBoosting & MLP\\
StandardScaler & AdaBoost & MultinomialNB\\
LogScaler & DecisionTree & GaussianNB\\
DataBalancer\\
\hline
 \end{tabular}
\end{table}

\begin{table}[h]
 \centering
 \footnotesize
 \caption{List of Meta-Features}
 \label{tbl:meta-features}
 \begin{tabular}{p{3cm}p{4cm}}
 \hline
 Property & Metric \\
 \hline \hline
Shape of Dataset & Number of rows and columns\\
Column types  & Presence of numeric, string category, Text, and date columns\\
Measure of symmetry & Skewness and Kurtosis\\
Measure of Distribution & Normal and Poisson\\
Tendency and Dispersion & Normalized mean and standard deviation\\
Balance of classes & Entropy \\
Correlation among columns & Pearson correlation\\
\hline
 \end{tabular}
\end{table}

\begin{definition}[Meta-feature]
\label{def:meta-feature}
meta-feature
\end{definition}

==> pipeline-grammar.tex <==
\setlength{\grammarparsep}{1px}
\grammarindent=56pt
\AtBeginEnvironment{grammar}{\footnotesize}
\begin{figure}
\begin{grammar}

<preprocessing> $\rightarrow$ <column\_loop>? <declare> <fit> <transform>

<column\_loop> $\rightarrow$ for col in <name>+:

<declare> $\rightarrow$ p = <name>()

<fit> $\rightarrow$ X[col] = p.fit\_transform(X[col]) | 
                    X = p.fit\_transform(X)

<transform> $\rightarrow$ y[col] = p.transform(y[col]) | 
                    y = p.transform(y)


<model> $\rightarrow$ m = <name>() \\
                        m.fit (X\_train, y\_train) \\
                        $y\_\textit{pred}$ = $m$.predict (X\_test)
                        

<name> $\rightarrow$ pre-processing component | model | column name

\end{grammar}
\caption{\label{fig:grammar} Grammar for preprocessing \& model components}
\end{figure}
